Distilling 3D distinctive local descriptors for 6D pose estimation

Three-dimensional local descriptors are crucial for encoding geometric surface properties, making them essential for various point cloud understanding tasks. Among these descriptors, GeDi has demonstrated strong zero-shot 6D pose estimation capabilities but remains computationally impractical for real-world applications due to its expensive inference process. Can we retain GeDi's effectiveness while significantly improving its efficiency? In this paper, we explore this question by introducing a knowledge distillation framework that trains an efficient student model to regress local descriptors from a GeDi teacher. Our key contributions include: an efficient large-scale training procedure that ensures robustness to occlusions and partial observations while operating under compute and storage constraints, and a novel loss formulation that handles weak supervision from non-distinctive teacher descriptors. We validate our approach on five BOP Benchmark datasets and demonstrate a significant reduction in inference time while maintaining competitive performance with existing methods, bringing zero-shot 6D pose estimation closer to real-time feasibility. Project Website: https://tev-fbk.github.io/dGeDi/

==> main/figures/block_diagram.tex <==

\begin{figure}[t!]
    \centering
    \resizebox{1\columnwidth}{!}{%
    \begin{overpic}[trim=20 28 15 15]
    {main/figures/block_diagram.pdf}
    \end{overpic}}

    \vspace{-0mm}
    \caption{
    \fabiocomment{optimise diagram to reduce empty spaces}
An Overview of~\acronym. Top: A Query point cloud is being fed to both teacher and student network. We obtain distinctive 3D local descriptor from (frozen) teacher which guide the student descriptors via proposed distillation loss. Bottom: Rather then computing the teacher features for Target objects, we leverage the learning via correspondences. We transfer the features from query to target point cloud using the ground-truth transformation available at training time. By leveraging this, we significantly reduce the memory and compute overhead.
    }
    \label{fig:comput_vs_transf}
    
\end{figure}

==> main/figures/computed_vs_transfered.tex <==
\begin{figure}[t!]
    \centering
    \resizebox{0.7\columnwidth}{3.9cm}{%
    \begin{overpic}[trim=0 0 5 0]{main/figures/computed_vs_transfered_crop.pdf}
    \end{overpic}}

    \vspace{0mm}
    \caption{
Top: Query Features, Bottom : (Left) Features computed on Target Object. (Right) : Features transferred to Target via ground truth correspondences.
    }
    \label{fig:comput_vs_transf}
\end{figure}

==> main/figures/losses.tex <==

% \begin{figure}[t!]
% \centerline{\includesvg[width=\columnwidth]{main/figures/losses.svg}}
% \caption{Loss curves for Huber, $L_1$ and $L_2$ }
% \label{fig: losses}
% \end{figure}


\begin{figure}[t!]
\begin{tikzpicture}
\begin{axis}[
    width=\columnwidth,
    height=7cm,
    xlabel={Error (pred - target)},
    ylabel={Loss Value},
    xmin=0, xmax=1,
    ymin=0, ymax=1,
    grid=major,
    legend style={at={(0.02,0.98)}, anchor=north west},
]

%------------------------------------------------
%% plot 1
%------------------------------------------------

\addplot [domain=0:0.3, samples=51, thick, color=blue] {0.5*x^2};
\addplot [domain=0.3:1, samples=51, thick, color=blue, forget plot] {0.3*(x - 0.15)};
\addlegendentry{$L_{\text{huber}}$}


%------------------------------------------------
% plot 2
%------------------------------------------------
\addplot [domain=0:0.3, samples=51, thick, color=orange] {
    (( (x+1e-6)^15 ) * (0.5*x^2)) / ((x+1e-6)^15 + 1e-6)
};

\addplot [domain=0.3:1, samples=51, thick, color=orange, forget plot] {
    (( (x+1e-6)^15 ) * (0.3*(x - 0.15))) / ((x+1e-6)^15 + 1e-6)
};
\addlegendentry{$L_{1}$}  % 

%------------------------------------------------
% plot 3
%------------------------------------------------
\addplot [domain=0:0.3, samples=51, thick, color=green!60!black] {8*x^2};
\addplot [domain=0.3:1, samples=51, thick, color=green!60!black, forget plot] {0.2*x + 0.66};
\addlegendentry{$L_{2}$}
\end{axis}

\end{tikzpicture}
\caption{
\fabiocomment{too much space this graph, shrink or remove.}
Comparison of loss functions: Huber loss ($L_{\text{huber}}$), Scaled-varient ($L_1$) loss, and proposed ($L_2$) loss across the error range $[0,1]$.}
\label{fig:losses}

\end{figure}


==> main/figures/pipeline.tex <==
\begin{figure*}[t!]
    \centering
    \begin{overpic}[trim=60 5 40 5, width=1\textwidth]{main/figures/pipeline.pdf}
    \end{overpic}

    \vspace{-3mm}
    \caption{Object 6D pose estimation pipeline used in our work.
    \fabiocomment{no need for this figure, just keep fig 3}
    }
    \label{fig:pipeline}
\end{figure*}

==> main/sections/todo.tex <==
\section{TODO}

\begin{itemize}
\item Distil the knowledge of PoZe~\cite{caraffa23poze} (teacher) with a WaffleIron-based~\cite{puy23waffleiron} neural network (student);
\item Predict a (calibrated) confidence score associated to the point-wise features;
\item Compare with MinkowskyEngine-based architectures;
\item Reduce the dimensionality of PoZe features;
\item Try different training data, e.g. MegaPose, ObjaVerse;
\item Consider using MixUp to fuse query and target objects (and the corresponding target features) in the same data sample;
\item Can we create a mixed mini-batch with both query and target objects? Or is it better to have two separate mini-batches?
\end{itemize}


==> main/tables/teacher2.tex <==
\begin{table}[t]
\renewcommand{\arraystretch}{0.9}
    \centering
    \tabcolsep 5pt
    \caption{
    Comparison of GeDi and \acronym on the BOP Benchmark in terms of feature quality (RON, FMR) and pose estimation accuracy (AR) with \textbf{GT} and \textbf{SAM6D} Masks. Reported time(Seconds) is for descriptor extraction only.
    Row~25,26 highlights \acronym improvement over GeDi.
    % \fabiocomment{indicate that Seconds in the table is for the feature extraction part}
    }
    \label{tab:teacher}
    \vspace{-3mm}
    \resizebox{\columnwidth}{!}{%
    \begin{tabular}{llcccc}

        \toprule
        & Dataset & RON {\color{gray}$\uparrow$} & FMR {\color{gray}$\uparrow$} & AR {\color{gray}$\uparrow$} & Seconds {\color{gray}$\downarrow$} \\
        \midrule
        \multicolumn{6}{c}{GeDi~\cite{poiesi2023gedi}} \\
        {\color{gray}\scriptsize 1} &\multirow{2}{*}{LM-O} & GT    & 1.8 & 8.8  & 66.9 & \multirow{2}{*}{3.198} \\
        {\color{gray}\scriptsize 3}& \multirow{2}{*}{T-LESS} & GT    & 0.4 & 1.0  & 44.5 & \multirow{2}{*}{3.600} \\
        {\color{gray}\scriptsize 5}& \multirow{2}{*}{TUD-L}  & GT    & 8.2 & 75.5 & 96.8 & \multirow{2}{*}{0.604} \\
         {\color{gray}\scriptsize 7}&\multirow{2}{*}{IC-BIN} & GT    & 1.0 & 11.6 & 31.9 & \multirow{2}{*}{6.126} \\
         {\color{gray}\scriptsize 9}&\multirow{2}{*}{YCB-V}  & GT    & 3.6 & 25.8 & 59.1 & \multirow{2}{*}{2.892} \\
          {\color{gray}\scriptsize 11}& \multirow{2}{*}{Avg}    & GT    & 3.0 & 24.5 & 59.8 & \multirow{2}{*}{3.284} \\
        \midrule
        \multicolumn{7}{c}{\acronym (ours)} \\
          {\color{gray}\scriptsize 13}& \multirow{2}{*}{LM-O}   & GT    & 4.3 & 27.2 & 67.2 & \multirow{2}{*}{0.021} \\
           {\color{gray}\scriptsize 14}&                      & SAM6D & 1.7 & 23.5 & 60.4 & \\
          {\color{gray}\scriptsize 15}& \multirow{2}{*}{T-LESS} & GT    & 2.1 & 15.6 & 58.6 & \multirow{2}{*}{0.021} \\
             {\color{gray}\scriptsize 16}&                    & SAM6D & 1.6 & 11.6 & 31.6 & \\
          {\color{gray}\scriptsize 17}& \multirow{2}{*}{TUD-L}  & GT    & 16.3 & 77.8 & 93.2 & \multirow{2}{*}{0.003} \\
            {\color{gray}\scriptsize 18}&                     & SAM6D & 12.8 & 67.3 & 83.0 & \\
          {\color{gray}\scriptsize 19}& \multirow{2}{*}{IC-BIN} & GT    & 3.7 & 18.5 & 33.1 & \multirow{2}{*}{0.034} \\
             {\color{gray}\scriptsize 20}&                    & SAM6D & 4.5 & 2.6  & 31.3 & \\
         {\color{gray}\scriptsize 21}&  \multirow{2}{*}{YCB-V}  & GT    & 9.1 & 42.3 & 58.8 & \multirow{2}{*}{0.015} \\
            {\color{gray}\scriptsize 22}&                     & SAM6D & 7.4 & 34.8 & 52.3 & \\
          {\color{gray}\scriptsize 23}& \multirow{2}{*}{Avg}    & GT    & \textbf{7.1} & \textbf{36.3} & \textbf{62.2} & \multirow{2}{*}{0.019} \\
            {\color{gray}\scriptsize 24}&                     & SAM6D & \textbf{5.6} & \textbf{27.9} & 51.7 & \\
        \midrule
         {\color{gray}\scriptsize 25}&\multirow{2}{*}{\scriptsize $\Delta$} & GT  & \color{forestgreen}\textbf{+4.1} & \color{forestgreen}\textbf{+11.8} & \color{forestgreen}\textbf{+2.4} & \multirow{2}{*}{\color{forestgreen}\textbf{170$\times$}} \\ 
         {\color{gray}\scriptsize 26} & & SAM6D & \color{forestgreen}\textbf{+2.7} & \color{forestgreen}\textbf{+9.4} & \color{red}\textbf{-1.1}  &  \\
        \midrule
        \multicolumn{7}{c}{GeDi~\cite{poiesi2023gedi}} \\
        {\color{gray}\scriptsize 1} &\multirow{2}{*}{LM-O} & GT    & 1.8 & 8.8  & 66.9 & \multirow{2}{*}{3.198} \\
        {\color{gray}\scriptsize 2} &                      & SAM6D & 3.5 & 7.4  & 60.7 & \\
        {\color{gray}\scriptsize 3}& \multirow{2}{*}{T-LESS} & GT    & 0.4 & 1.0  & 44.5 & \multirow{2}{*}{3.600} \\
          {\color{gray}\scriptsize 4} &                   & SAM6D & 0.4 & 0.7  & 31.6 & \\
        {\color{gray}\scriptsize 5}& \multirow{2}{*}{TUD-L}  & GT    & 8.2 & 75.5 & 96.8 & \multirow{2}{*}{0.604} \\
          {\color{gray}\scriptsize 6}  &                  & SAM6D & 6.6 & 58.6 & 89.5 & \\
         {\color{gray}\scriptsize 7}&\multirow{2}{*}{IC-BIN} & GT    & 1.0 & 11.6 & 31.9 & \multirow{2}{*}{6.126} \\
          {\color{gray}\scriptsize 8}  &                  & SAM6D & 0.6 & 1.8  & 29.0 & \\
         {\color{gray}\scriptsize 9}&\multirow{2}{*}{YCB-V}  & GT    & 3.6 & 25.8 & 59.1 & \multirow{2}{*}{2.892} \\
          {\color{gray}\scriptsize 10}&                    & SAM6D & 3.2 & 23.7 & 53.0 & \\
          {\color{gray}\scriptsize 11}& \multirow{2}{*}{Avg}    & GT    & 3.0 & 24.5 & 59.8 & \multirow{2}{*}{3.284} \\
            {\color{gray}\scriptsize 12}&                     & SAM6D & 2.9 & 18.5 & \textbf{52.8} & \\
        \midrule
        \multicolumn{7}{c}{\acronym (ours)} \\
          {\color{gray}\scriptsize 13}& \multirow{2}{*}{LM-O}   & GT    & 4.3 & 27.2 & 67.2 & \multirow{2}{*}{0.021} \\
           {\color{gray}\scriptsize 14}&                      & SAM6D & 1.7 & 23.5 & 60.4 & \\
          {\color{gray}\scriptsize 15}& \multirow{2}{*}{T-LESS} & GT    & 2.1 & 15.6 & 58.6 & \multirow{2}{*}{0.021} \\
             {\color{gray}\scriptsize 16}&                    & SAM6D & 1.6 & 11.6 & 31.6 & \\
          {\color{gray}\scriptsize 17}& \multirow{2}{*}{TUD-L}  & GT    & 16.3 & 77.8 & 93.2 & \multirow{2}{*}{0.003} \\
            {\color{gray}\scriptsize 18}&                     & SAM6D & 12.8 & 67.3 & 83.0 & \\
          {\color{gray}\scriptsize 19}& \multirow{2}{*}{IC-BIN} & GT    & 3.7 & 18.5 & 33.1 & \multirow{2}{*}{0.034} \\
             {\color{gray}\scriptsize 20}&                    & SAM6D & 4.5 & 2.6  & 31.3 & \\
         {\color{gray}\scriptsize 21}&  \multirow{2}{*}{YCB-V}  & GT    & 9.1 & 42.3 & 58.8 & \multirow{2}{*}{0.015} \\
            {\color{gray}\scriptsize 22}&                     & SAM6D & 7.4 & 34.8 & 52.3 & \\
          {\color{gray}\scriptsize 23}& \multirow{2}{*}{Avg}    & GT    & \textbf{7.1} & \textbf{36.3} & \textbf{62.2} & \multirow{2}{*}{0.019} \\
            {\color{gray}\scriptsize 24}&                     & SAM6D & \textbf{5.6} & \textbf{27.9} & 51.7 & \\
        \midrule
         {\color{gray}\scriptsize 25}&\multirow{2}{*}{\scriptsize $\Delta$} & GT  & \color{forestgreen}\textbf{+4.1} & \color{forestgreen}\textbf{+11.8} & \color{forestgreen}\textbf{+2.4} & \multirow{2}{*}{\color{forestgreen}\textbf{170$\times$}} \\ 
         {\color{gray}\scriptsize 26} & & SAM6D & \color{forestgreen}\textbf{+2.7} & \color{forestgreen}\textbf{+9.4} & \color{red}\textbf{-1.1}  &  \\
\bottomrule




        
    \end{tabular}
    }
\end{table}










%%% table backup
% \begin{table}[t]
%     \centering
%     \tabcolsep 5pt
%     \caption{
%     Comparison of GeDi and \acronym on the BOP Benchmark in terms of feature quality (RON, FMR), pose estimation accuracy (AR) with \textbf{GT/SAM6D} Masks, Reported time is for descriptor extraction.
%     Row~13 highlights \acronym improvement over GeDi.
%     }
%     \label{tab:teacher}

%     \vspace{-3mm}
%     \resizebox{\columnwidth}{!}{%
%     \begin{tabular}{rlcccc}
%         \toprule
%         & Dataset & RON {\color{gray} $\uparrow$} & FMR {\color{gray} $\uparrow$} & AR {\color{gray} $\uparrow$} & Seconds {\color{gray} $\downarrow$} \\
%         \midrule
%         \multicolumn{6}{c}{GeDi~\cite{poiesi2023gedi}} \\
%         {\color{gray} \scriptsize 1} & LM-O & 1.8/3.5 & 8.8/7.4 & 66.9/60.7 & 3.198 \\
%         {\color{gray} \scriptsize 2} & T-LESS & 0.4/0.4 & 1.0/0.7 & 44.5/31.6 & 3.600 \\
%         {\color{gray} \scriptsize 3} & TUD-L & 8.2/6.6 & 75.5/58.6 & 96.8/89.5 & 0.604 \\
%         {\color{gray} \scriptsize 4} & IC-BIN & 1.0/0.6 & 11.6/1.8 & 31.9/29.0 & 6.126 \\
%         {\color{gray} \scriptsize 5} & YCB-V & 3.6/3.2 & 25.8/23.7 & 59.1/53.0 & 2.892 \\
%         {\color{gray} \scriptsize 6} & Avg & 3.0/2.9 & 24.5/18.5 & 59.8/\textbf{52.8} & 3.284 \\
%         \midrule
%         \multicolumn{6}{c}{\acronym (ours)} \\
%         {\color{gray} \scriptsize 7} & LM-O & 4.3/1.7 & 27.2/23.5 & 67.2/60.4 & 0.021 \\
%         {\color{gray} \scriptsize 8} & T-LESS & 2.1/1.6 & 15.6/11.6 & 58.6/31.6 & 0.021 \\
%         {\color{gray} \scriptsize 9} & TUD-L & 16.3/12.8 & 77.8/67.3 & 93.2/83.0 & 0.003 \\
%         {\color{gray} \scriptsize 10} & IC-BIN & 3.7/4.5 & 18.5/2.6 & 33.1/31.3 & 0.034 \\
%         {\color{gray} \scriptsize 11} & YCB-V & 9.1/7.4 & 42.3/34.8 & 58.8/52.3 & 0.015 \\
%         {\color{gray} \scriptsize 12} & Avg & \textbf{7.1}/\textbf{5.6} & \textbf{36.3}/\textbf{27.9} & \textbf{62.2}/51.7 & \textbf{0.019} \\
%         \midrule
%         {\color{gray} \scriptsize 13} & $\Delta$ & \color{forestgreen}\textbf{+4.1}/\color{forestgreen}\textbf{+2.7} & \color{forestgreen}\textbf{+11.8}/\color{forestgreen}\textbf{+9.4} & \color{forestgreen}\textbf{+2.4}/\color{red}\textbf{-1.1} & \color{forestgreen}\textbf{170$\times$} \\
%         \bottomrule
%     \end{tabular}
%     }
% \end{table}


==> main/tables/teacher_orizzontal.tex <==
\begin{table*}[t]
    \centering
    % \tabcolsep 2pt
    \caption{
    Comparison of GeDi and \acronym on the BOP Benchmark in terms of 3D registration accuracy (RON and FMR), 6D pose estimation accuracy (AR), and time required to process an image (Seconds).
    The last column highlights the student improvement over the teacher performance for each metric as absolute improvement in percentage points~(Rows 5-7) and speed-up factor~(Row 8).
    \fabiocomment{this table takes too much space, see if you can squeeze it in one column or some other way}
    }
    \label{tab:teacher}

    \vspace{-3mm}
    \resizebox{\textwidth}{!}{%
    \begin{tabular}{rllrrrrrrr}
        \toprule
        & Method & Metric & LM-O & T-LESS & TUD-L & IC-BIN & YCB-V & Avg & $\Delta$ \\
        \toprule
        {\color{gray} \scriptsize 1} & \multirow{4}{*}{GeDi~\cite{poiesi2023gedi}} & RON {\color{gray} $\uparrow$} & 1.8 & 0.4 & 8.2 & 1.0 & 3.6 & 3.0 & - \\
        {\color{gray} \scriptsize 2} & & FMR {\color{gray} $\uparrow$} & 8.8 &1.0 & 75.5 &11.6 & 25.8 & 24.5 & - \\
        % {\color{gray} \scriptsize 2} & & MNN {\color{gray} $\uparrow$} & 193 & 129 & 247 & 156 & 159 & \textbf{177} \\
        % {\color{gray} \scriptsize 2} & & MNN $<$ the $\downarrow$ & 4 & 1  & 20  &  2 & 6 & \textbf{7} \\
        {\color{gray} \scriptsize 3} & & AR {\color{gray} $\uparrow$} & 66.9 & 44.5 & 96.8 & 31.9 & 59.1 & 59.8 & - \\
        {\color{gray} \scriptsize 4} & & Seconds {\color{gray} $\downarrow$} & 3.198 & 3.600  & 0.604  & 6.126 & 2.892 & 3.284 & - \\
        % \midrule
        % {\color{gray} \scriptsize 4} & \multirow{3}{*}{GeDi~\cite{poiesi2023gedi} (3-scales)} & Feat. qual. (MNNR) & \\
        % {\color{gray} \scriptsize 5} & & Time (s) & 9.762 & 10.788 & 1.713 & 17.831 & 9.103 & -- \\
        % {\color{gray} \scriptsize 6} & & Accuracy (AR) & 71.2 & 45.6 & 97.5 & 32.1 & 59.2  & 61.1 \\
        \midrule
        {\color{gray} \scriptsize 5} & \multirow{4}{*}{\acronym (ours)} & RON {\color{gray} $\uparrow$} & 4.3 & 2.1 & 16.3 & 3.7 & 9.1 & \textbf{7.1} & \textcolor{ForestGreen}{+4.1} \\
        {\color{gray} \scriptsize 6} & & FMR {\color{gray} $\uparrow$} & 27.2 &15.6 & 77.8 &18.5 & 42.3 & \textbf{36.3} & \textcolor{ForestGreen}{+11.8} \\
        % {\color{gray} \scriptsize 6} & 
        % \multirow{5}{*}{\acronym (ours)} & MNN $\uparrow$ & 68 & 64 & 93 & 47 & 75 & 70 \\
        % {\color{gray} \scriptsize 7} & & MNN $<$ the $\downarrow$ & 4 &  3 & 18  & 3  & 10 & \textbf{7} \\
        {\color{gray} \scriptsize 7} & & AR {\color{gray} $\uparrow$} & 67.2 & 58.6 & 93.2 & 33.1 & 58.8 & \textbf{62.2} & \textcolor{ForestGreen}{+2.4} \\
        {\color{gray} \scriptsize 8} & & Seconds {\color{gray} $\downarrow$} & 0.021 & 0.021 & 0.003 & 0.034 & 0.015 & \textbf{0.019} & \textcolor{ForestGreen}{170$\times$} \\
        \bottomrule
    \end{tabular}
    }
\end{table*}



%  %--- LMO ---
%  LMO   & 193 & 4 & 1.8   & 68 & 4 & 4.3 \\
%  %--- TLESS ---
%  TLESS & 129 & 1 & 0.4   & 64 & 3 & 2.1 \\
%  %--- TUD-L ---
%  TUD-L & 247 & 20 & 8.2  & 93 & 18 & 16.3 \\
%  %--- ICBIN ---
%  ICBIN & 156 & 2 & 1.0   & 47 & 3 & 3.7 \\
%  %--- YCBV ---
%  YCBV  & 159 & 6 & 3.6   & 75 & 10 & 9.1 \\
% \midrule
%  % -- Average ---
%  Average  & 177 & 7 & 3.0   & 70 & 7 & 7.1 \\
